S-Agents: Self-organizing Agents in Open-ended Environments

Leveraging large language models (LLMs), autonomous agents have significantly improved, gaining the ability to handle a variety of tasks. In open-ended settings, optimizing collaboration for efficiency and effectiveness demands flexible adjustments. Despite this, current research mainly emphasizes fixed, task-oriented workflows and overlooks agent-centric organizational structures. Drawing inspiration from human organizational behavior, we introduce a self-organizing agent system (S-Agents) with a "tree of agents" structure for dynamic workflow, an "hourglass agent architecture" for balancing information priorities, and a "non-obstructive collaboration" method to allow asynchronous task execution among agents. This structure can autonomously coordinate a group of agents, efficiently addressing the challenges of open and dynamic environments without human intervention. Our experiments demonstrate that S-Agents proficiently execute collaborative building tasks and resource collection in the Minecraft environment, validating their effectiveness.

==> figures/7-exp.tex <==
\begin{figure*}[t]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{figures/7_exp.pdf}
	\end{center}
\vspace{-1em}
	\caption{
\textbf{Collaborative collection:} 
%
\textbf{(a)} Efficiency of three agents mining 50 stones under different organizational structures; 
%
CoA and GoA each consist of 3 agents, where \texttt{ToA(n)} represents an agent organization with one root and \texttt{n} leaves.
%
Due to the presence of command cycle issues in GoA, the planning module, which utilized gpt-3.5-turbo-16k, was upgraded to gpt-4 for experimentation.
%
\textbf{(b)} Time cost (/min) of 1, 2, and 3 agents on various tasks, \texttt{NaN} denotes no progress for over 40 minutes. 
% 
\textbf{(c)} Efficiency comparison (time cost/min) between multi-agent and solo agent across different task difficulties.}
 \vspace{-1em}
	\label{fig:exp}
\end{figure*}
